A High-Performance Implementation of a Robust Preconditioner for Heterogeneous Problems

We present an efficient implementation of the highly robust and scalable GenEO preconditioner in the high-performance PDE framework DUNE. The GenEO coarse space is constructed by combining low energy solutions of a local generalised eigenproblem using a partition of unity. In this paper we demonstrate both weak and strong scaling for the GenEO solver on over 15,000 cores by solving an industrially motivated problem with over 200 million degrees of freedom. Further, we show that for highly complex parameter distributions arising in certain real-world applications, established methods become intractable while GenEO remains fully effective. The purpose of this paper is two-fold: to demonstrate the robustness and high parallel efficiency of the solver and to document the technical details that are crucial to the efficiency of the code.

==> multiscale.tex <==
 

\section{GenEO as Multiscale Method}

In highly heterogeneous problems, a simple coarse space may not represent
local coefficient variations that, while only occuring in small scale, may
still strongly affect the large-scale solution. In order to resolve these
coefficient changes, one can choose a fine resolution of the finite element
discretization. However, this easily increases computational effort beyond
available capacities. Another option would be to instead incorporate these
coefficient jumps in the coarse basis, thereby resolving the small-scale
variations without needing to introduce a large number of additional degrees
of freedom.

This approach is referred to as generalized multiscale finite element method
(GMsFEM) and has been proven to be effective in {\cite{BabuskaLipton}} for a
different choice of basis functions. While such a basis can be tailored
specifically to the problem at hand as shown in {\cite{BabuskaCalozOsborn}},
this construction may be extremely difficult in all but very simple problems.
Using the result of a generalized Eigenproblem removes the need for prior
knowledge about the problem's structure, rendering the GenEO space an
attractive option as an efficient problem-specific coarse basis. The GenEO space
could successfully be applied in such a way in {\cite{CustomizedCoarseModels}}
and in section \ref{GenEOSpectralBasis}.

\subsection{Solving in the Coarse Space}

In this setting, solving this coarse problem boils down to
\[ x = R_H^T ( A_H)^{- 1} R_H b, \]
where $A_H$ is the coarse system from GenEO and $b$ is the right hand side of
the discrete problem to be solved. Note that in contrast to using the GenEO
coarse space in a two-level Schwarz method, no local subdomain solves are
performed and only a single coarse solve is needed. Even though a larger
coarse space may be necessary, as long as the approximation is sufficient,
this approach may offer a large decrease in computational effort.



Obviously, if more eigenvectors are chosen in the GenEO coarse space, the
approximation of the solution improves. However, as the numerical results in
section \ref{GenEOSpectralBasisApprox} indicate, this approach can already
deliver a surprisingly good approximation with only a very small basis if the
GenEO basis represents the problem well.

\begin{corollary}

The coarse approximation error is bounded by

\begin{eqnarray*}
  \| v - v_H \|_{a, \Omega}
  \leqslant k_0  \left( 1 + \frac{1}{\underset{j}{\min} \, \lambda_{m_j +
  1}} \right)^{\frac{1}{2}} | v |_{a, \Omega}.
\end{eqnarray*}

\begin{proof}

In the setting of Lemma \ref{StableSplitting}, this follows by extending the
estimate (\ref{StableSplitIneq}) to the entire domain $\Omega$.

\begin{eqnarray*}
  \| v - v_H \|_{a, \Omega} & = & \left\| \sum_{j = 1}^N \Xi_j  ( v |
  \nobracket_{\Omega_j} - \Pi_{m_j}^j v | \nobracket_{\Omega_j}) \right\|_{a,
  \Omega}\\
  & = & \left\| \sum_{j = 1}^N z_j \right\|_{a, \Omega}\\
  & \leqslant & \sum_{j = 1}^N \| z_j \|_{a, \Omega_j}\\
  & \leqslant & \sum_{j = 1}^N  \left( 1 + \frac{1}{\lambda_{m_j + 1}^j}
  \right)^{\frac{1}{2}} | v |_{a, \Omega_j}\\
  & \leqslant & k_0  \left( 1 + \frac{1}{\underset{j}{\min} \, \lambda_{m_j +
  1}} \right)^{\frac{1}{2}} | v |_{a, \Omega}.
\end{eqnarray*}
\end{proof}
\end{corollary}

\todo[inline]{Lipton/Babuska theory applicable?}

Clearly, quality of the approximation directly depends on the eigenvalues from
the generalized eigenproblem. For a small number of near-zero eigenvalues far
apart from the following larger ones, the approximation yields the best results.


\subsection{GenEO Basis on Highly Structured Problems}

\begin{figure}[t]
 \centering

\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=.6\linewidth]{"Problem2_Parameters".png}
  \caption{Parameter distribution and domain decomposition}
  \label{CoarseApproxErrorSkyscrapers:sub1}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=.6\linewidth]{"Coarse Error Problem2 1EV".png}
  \caption{1 EV per subdomain}
  \label{CoarseApproxErrorSkyscrapers:sub2}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=.6\linewidth]{"Coarse Error Problem2 2EV".png}
  \caption{2 EVs per subdomain}
  \label{CoarseApproxErrorSkyscrapers:sub3}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=.6\linewidth]{"Coarse Error Problem2 3EV".png}
  \caption{3 EV per subdomain}
  \label{CoarseApproxErrorSkyscrapers:sub4}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=.6\linewidth]{"Coarse Error Problem2 4EV".png}
  \caption{4 EV per subdomain}
  \label{CoarseApproxErrorSkyscrapers:sub5}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=.6\linewidth]{"Coarse Error Problem2 5EV".png}
  \caption{5 EV per subdomain}
  \label{CoarseApproxErrorSkyscrapers:sub6}
\end{subfigure}

 \caption{Coarse approximation error}
 \label{CoarseApproxErrorSkyscrapers}
\end{figure}

With clearly structured problems, it can be visually seen that the GenEO coarse space
systematically picks up inclusions or channels in the parameter distribution.

In figure \ref{CoarseApproxErrorSkyscrapers} the coarse approximation error is shown
for a Darcy problem with Dirichlet conditions set to one at the top and zero at the bottom,
Neumann conditions at the remaining boundary and a high-contrast parameter distribution
as shown in \ref{CoarseApproxErrorSkyscrapers:sub1}.

As can be seen in figure \ref{CoarseApproxErrorSkyscrapers:sub1}, each inclusion has an effect
on the approximation error. Adding one additional eigenvector from each subdomain to the
coarse basis removes some of those error sources (\ref{CoarseApproxErrorSkyscrapers:sub2}).
The next eigenvectors pick up the skyscrapers (\ref{CoarseApproxErrorSkyscrapers:sub3}), in
(\ref{CoarseApproxErrorSkyscrapers:sub4}) most channels are picked up and the last remaining
channel section not captured so far is picked up in (\ref{CoarseApproxErrorSkyscrapers:sub5}).

So, in this particular example, a total of 25 coarse basis functions is enough to almost entirely solve
the given problem.

\subsection{Comparison to Lipton-Babuska Coarse Space}

\todo[inline]{Finish implementation/testing, comparison}

\subsection{Approximation of Linear Elasticity Problems}

\todo[inline]{dune-composites with coarse solution vs basis size}


==> preconditioner.tex <==
 

\subsection{Robustness}


\begin{figure}[t]
 \centering
 \includegraphics[scale=0.4]{Darcy_Iso_Layers_Contrast.eps}
 \caption{Robustness of GenEO preconditioner with respect to parameter contrast}
\end{figure}

\begin{figure}[t]
 \centering
 \includegraphics[scale=0.4]{Darcy_Iso_3D_Layers_Subdomains_Condition.eps}
 \caption{Robustness of GenEO preconditioner with respect to parameter contrast}
\end{figure}

